Improving Compound Activity Classification via Deep Transfer and Representation Learning

Recent advances in molecular machine learning, especially deep neural networks such as Graph Neural Networks (GNNs) for predicting structure activity relationships (SAR) have shown tremendous potential in computer-aided drug discovery. However, the applicability of such deep neural networks are limited by the requirement of large amounts of training data. In order to cope with limited training data for a target task, transfer learning for SAR modeling has been recently adopted to leverage information from data of related tasks. In this work, in contrast to the popular parameter-based transfer learning such as pretraining, we develop novel deep transfer learning methods TAc and TAc-fc to leverage source domain data and transfer useful information to the target domain. TAc learns to generate effective molecular features that can generalize well from one domain to another, and increase the classification performance in the target domain. Additionally, TAc-fc extends TAc by incorporating novel components to selectively learn feature-wise and compound-wise transferability. We used the bioassay screening data from PubChem, and identified 120 pairs of bioassays such that the active compounds in each pair are more similar to each other compared to its inactive compounds. Our experiments clearly demonstrate that TAc achieves significant improvement over all baselines across a large number of target tasks. Furthermore, although TAc-fc achieves slightly worse ROC-AUC on average compared to TAc, TAc-fc still achieves the best performance on more tasks in terms of PR-AUC and F1 compared to other methods. In summary, TAc-fc is also found to be a strong model with competitive or even better performance than TAc on a notable number of target tasks.

==> define.tex <==
% methods
\newcommand{\RankMethod}{\mbox{$\mathop{\mathtt{gnnCP}}\limits$}\xspace}
\newcommand{\OurMethod}{\mbox{$\mathop{\mathtt{TAc}}\limits$}\xspace}
\newcommand{\OurMethodWithDisc}{\mbox{$\mathop{\mathtt{TAc\text{-}fc}}\limits$}\xspace}

\newcommand{\OurMethodWithLocalDisc}{\mbox{$\mathop{\mathtt{TAc\text{-}f}}\limits$}\xspace}
\newcommand{\OurMethodWithGlobalDisc}{\mbox{$\mathop{\mathtt{TAc\text{-}c}}\limits$}\xspace}

\newcommand{\OurMethodWithDMPNNAWithLocalDisc}{\mbox{$\mathop{\mathtt{TAc\text{-}f\text{-}\newgnn}}\limits$}\xspace}
\newcommand{\OurMethodWithDMPNNAWithGlobalDisc}{\mbox{$\mathop{\mathtt{TAc\text{-}c\text{-}\newgnn}}\limits$}\xspace}

\newcommand{\OurMethodWithDMPNN}{\mbox{$\mathop{\OurMethod\text{-}\dmpnn}\limits$}\xspace}
\newcommand{\OurMethodWithDMPNNA}{\mbox{$\mathop{\OurMethod\text{-}\newgnn}\limits$}\xspace}
\newcommand{\OurMethodWithDMPNNWithDisc}{\mbox{$\mathop{\OurMethodWithDisc\text{-}\dmpnn}\limits$}\xspace}
\newcommand{\OurMethodWithDMPNNAWithDisc}{\mbox{$\mathop{\OurMethodWithDisc\text{-}\newgnn}\limits$}\xspace}
\newcommand{\gnn}{\mbox{$\mathop{\mathtt{GNN}}\limits$}\xspace}
\newcommand{\gnns}{\mbox{$\mathop{\mathtt{GNNs}}\limits$}\xspace}

% baseline methods
\newcommand{\morganFCN}{\mbox{$\mathop{\mathtt{FCN}\text{-}\mathtt{morgan}}\limits$}\xspace}
\newcommand{\morgancFCN}{\mbox{$\mathop{\mathtt{FCN}\text{-}\mathtt{morganc}}\limits$}\xspace}
\newcommand{\dmpnnFCN}{\mbox{$\mathop{\mathtt{FCN}\text{-}\mathtt{\dmpnn}}\limits$}\xspace}
\newcommand{\newgnnFCN}{\mbox{$\mathop{\mathtt{FCN}\text{-}\mathtt{\newgnn}}\limits$}\xspace} 

% data transfer baselines
\newcommand{\dmpnnFCNDT}{\mbox{$\mathop{\mathtt{FCN}\text{-}\mathtt{\dmpnn} ~(\datatransfer)}\limits$}\xspace}
\newcommand{\newgnnFCNDT}{\mbox{$\mathop{\mathtt{FCN}\text{-}\mathtt{\newgnn} ~(\datatransfer)}\limits$}\xspace} 

% transfer learning baselines
\newcommand{\DANN}{\mbox{$\mathop{\mathtt{DANN}}\limits$}\xspace}
\newcommand{\DANNWithDMPNN}{\mbox{$\mathop{\DANN\text{-}\dmpnn}\limits$}\xspace}
\newcommand{\DANNWithDMPNNA}{\mbox{$\mathop{\DANN\text{-}\newgnn}\limits$}\xspace}

% experimental setting 
\newcommand{\datatransfer}{\mbox{$\mathop{\mathtt{DT}}\limits$}\xspace}
\newcommand{\notransfer}{\mbox{$\mathop{\mathtt{noT}}\limits$}\xspace}

% source and target tasks
\newcommand{\SourceDomain}{\mbox{$\mathop{\mathcal{D}^{(S)}}\limits$}\xspace}
\newcommand{\TargetDomain}{\mbox{$\mathop{\mathcal{D}^{(T)}}\limits$}\xspace}
\newcommand{\SourceTask}{\mbox{$\mathop{\mathcal{T}^{(S)}}\limits$}\xspace}
\newcommand{\TargetTask}{\mbox{$\mathop{\mathcal{T}^{(T)}}\limits$}\xspace}

\newcommand{\source}{\mbox{$\mathop{\mathtt{Src}}\limits$}\xspace}
\newcommand{\target}{\mbox{$\mathop{\mathtt{Tgt}}\limits$}\xspace}

% metrics
\newcommand{\prauc}{\mbox{$\mathop{\mathtt{PR\text{-}AUC}}\limits$}\xspace}
\newcommand{\rocauc}{\mbox{$\mathop{\mathtt{ROC\text{-}AUC}}\limits$}\xspace}
\newcommand{\precision}{\mbox{$\mathop{\mathtt{precision}}\limits$}\xspace}
\newcommand{\recall}{\mbox{$\mathop{\mathtt{recall}}\limits$}\xspace}
\newcommand{\sensitivity}{\mbox{$\mathop{\mathtt{sens}}\limits$}\xspace}
\newcommand{\specificity}{\mbox{$\mathop{\mathtt{specificity}}\limits$}\xspace}
\newcommand{\tnr}{\mbox{$\mathop{\mathtt{TNR}}\limits$}\xspace}
\newcommand{\accuracy}{\mbox{$\mathop{\mathtt{accuracy}}\limits$}\xspace}
\newcommand{\fone}{\mbox{$\mathop{\mathtt{F1}}\limits$}\xspace}

%\newcommand{\method}{\mbox{$\mathop{\mathtt{M^2pht}}\limits$}\xspace}
\newcommand{\MPNN}{\mbox{$\mathop{\mathtt{MPNN}}\limits$}\xspace}
%\newcommand{\dmpnn}{\mbox{$\mathop{\mathtt{D\textrm{-}MPNN}}\limits$}\xspace}
\newcommand{\dmpnn}{\mbox{$\mathop{\mathtt{dmpn}}\limits$}\xspace}
%\newcommand{\Admpnn}{\mbox{$\mathop{\mathtt{A\textrm{-}dmpnn}}\limits$}\xspace}
\newcommand{\MORGAN}{\mbox{$\mathop{\mathtt{morgan}}\limits$}\xspace}
\newcommand{\MORGANC}{\mbox{$\mathop{\mathtt{morgan\textrm{-}c}}\limits$}\xspace}
\newcommand{\MORGANBA}{\mbox{$\mathop{\mathtt{morgan\textrm{-}ba}}\limits$}\xspace}
\newcommand{\RDKITGD}{\mbox{$\mathop{\mathtt{RDKit200}}\limits$}\xspace}
%\newcommand{\dmpnnDA}{\mbox{$\mathop{\mathtt{dmpnn\textrm{+}Disc}}\limits$}\xspace} %my method with dmpnn
%\newcommand{\AdmpnnDA}{\mbox{$\mathop{\mathtt{Admpnn\textrm{+}Disc}}\limits$}\xspace} % my method with A-dmpnn

\newcommand{\newgnn}{\mbox{$\mathop{\mathtt{dmpna}}\limits$}\xspace} 


% modules/components
\newcommand{\fgen}{\mbox{$\mathtt{F}$}\xspace}
\newcommand{\ldisc}{\mbox{$\mathtt{L}$}\xspace}
\newcommand{\gdisc}{\mbox{$\mathtt{G}$}\xspace}
\newcommand{\classifier}{\mbox{$\mathtt{S}$}\xspace}
\newcommand{\fatt}{\mbox{$f_a$}\xspace}

% parameters
\newcommand{\ParGnn}{\mbox{$\Omega$}\xspace}
\newcommand{\ParLdisc}{\mbox{$\Theta$}\xspace}
\newcommand{\ParGdisc}{\mbox{$\Psi$}\xspace}
\newcommand{\ParClassifier}{\mbox{$\Phi$}\xspace}

% compounds and graphs
\newcommand{\MolGraph}{\mbox{${\mathcal{G}}$}\xspace}
\newcommand{\compound}{\mbox{$c$}\xspace}
\newcommand{\bioassay}{\mbox{$B$}\xspace}
\newcommand{\SetAtoms}{\mbox{$\mathcal{A}$}\xspace}
\newcommand{\SetBonds}{\mbox{$\mathcal{E}$}\xspace}
\newcommand{\SetCompounds}{\mbox{$\mathcal{X}$}\xspace}
\newcommand{\SetLabels}{\mbox{$\mathcal{Y}$}\xspace}

\newcommand{\InputFeature}{\mbox{${\mathbf{x}}$}\xspace}
\newcommand{\Label}{\mbox{$y$}\xspace}
\newcommand{\AtomFeature}{\mbox{${\mathbf{a}}$}\xspace}
\newcommand{\BondFeature}{\mbox{${\mathbf{e}}$}\xspace}
\newcommand{\FeatureSpace}{\mbox{${\mathbb{X}}$}\xspace}
\newcommand{\LabelSpace}{\mbox{${\mathbb{Y}}$}\xspace}

\newcommand{\domain}{\mbox{${\mathcal{D}}$}\xspace}
\newcommand{\task}{\mbox{${\mathcal{T}}$}\xspace}
\newcommand{\entropy}{\mbox{${H}$}\xspace}

\newcommand{\embedding}{\mbox{${\mathbf{s}}$}\xspace}
\newcommand{\mes}{\mbox{${\mathbf{m}}$}\xspace}
\newcommand{\hidden}{\mbox{${\mathbf{h}}$}\xspace}
\newcommand{\compr}{\mbox{${\mathbf{r}}$}\xspace}
\newcommand{\scompr}{\mbox{${\mathbf{z}}$}\xspace}
%\newcommand{\ModifiedCompr}{\mbox{$\mathbf{z}$}\xspace}
\newcommand{\prob}{\mbox{$\mathbf{p}$}\xspace}
\newcommand{\params}{\mbox{$\Theta$}\xspace}

\newcommand{\FinalLoss}{\mbox{$\mathcal{L}$}\xspace}
\newcommand{\ClassifierLoss}{\mbox{$\mathcal{L}_{(c)}$}\xspace}
\newcommand{\LocalDiscLoss}{\mbox{$\mathcal{L}_{(l)}$}\xspace}
\newcommand{\GlobalDiscLoss}{\mbox{$\mathcal{L}_{(g)}$}\xspace}

%\newcommand{\onlyT}{\mbox{$\mathop{\mathtt{OT}}\limits$}\xspace}
%\newcommand{\SandT}{\mbox{$\mathop{\mathtt{S+T}}\limits$}\xspace}


\newcommand{\numImpv}{\mbox{$\mathop{\mathtt{N\textrm{-}impv}}\limits$}\xspace}
\newcommand{\taskImpv}{\mbox{$\mathop{\mathtt{t\textrm{-}impv\%}}\limits$}\xspace}
\newcommand{\diff}{\mbox{$\mathop{\mathtt{diff\%}}\limits$}\xspace}
\newcommand{\taskDiff}{\mbox{$\mathop{\mathtt{t\textrm{-}diff\%}}\limits$}\xspace}
\newcommand{\corr}{\mbox{$\mathop{\mathtt{corr}}\limits$}\xspace}
\newcommand{\pvalue}{\mbox{$\mathop{\mathtt{p\textrm{-}value}}\limits$}\xspace}
\newcommand{\simDiff}{\mbox{$\mathop{\mathtt{sdiff\%}}\limits$}\xspace}
\newcommand{\eSimDiff}{\mbox{$\mathop{\mathtt{e\textrm{-}sdiff\%}}\limits$}\xspace}


% issues in writing
\newcommand{\xia}[1]{\textcolor{red}{#1}}
\newcommand{\raghu}[1]{\textcolor{orange}{Raghu: #1}}
\newcommand{\vmodified}[1]{\textcolor{blue}{#1}}
\newcommand{\vcomments}[1]{\textcolor{cyan}{(#1)}}
\newcommand{\vnew}[1]{\textcolor{brown}{#1}}

==> figs/comp_viz.tex <==
\begin{figure*}[h!]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/compounds/TP-NP_000762-NP_000752.pdf}
        \caption{\scriptsize{A \emph{correctly} classified compound from the target bioassay NP\_000752 and its top-5 most similar compounds from the source bioassay NP\_000762}}
    \end{subfigure}
    
    
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/compounds/TP-NP_004337-NP_660205.pdf}
        \caption{\scriptsize{A \emph{correctly} classified compound from the target bioassay NP\_660205 and its top-5 most similar compounds from the source bioassay NP\_004337}}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/compounds/FN-NP_000762-NP_000752.pdf}
        \caption{\scriptsize{An \emph{incorrectly} classified compound from the target bioassay NP\_000752 and its top-5 most similar compounds from the source bioassay NP\_000762}}
    \end{subfigure}
    
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/compounds/FN-NP_004337-NP_660205.pdf}
         \caption{\scriptsize{An \emph{incorrectly} classified compound from the target bioassay NP\_660205 and its top-5 most similar compounds from the source bioassay NP\_004337}}
    \end{subfigure}

    \caption{Visualization of a few selected compounds from the target bioassay and their corresponding top-5 most similar compounds from the source bioassay.}
    \label{fig:compounds}
\end{figure*}


==> figs/param_study_best_tasks_aada_dmpnna_LG.tex <==
\begin{figure}[h!]
    \centering
        \includegraphics[width=0.3\textwidth]{figs/parameter_study/best_tasks_aada+dmpnna+L+G/mean-roc-auc.jpg}
      \caption{Parameter Study of \OurMethodWithDMPNNAWithDisc in terms of \rocauc}
    \label{fig:param_best_tasks_aada_dmpnna_LG}
\end{figure}


==> figs/perf_diff_similarity_matrix.tex <==
\begin{figure*}[h!]
    \centering
    \begin{subfigure}{0.26\textwidth}
        \centering
        \includegraphics[width=.9\textwidth]{figs/sim_matrix/NP_000676-NP_005152.jpg}
        \caption{\mbox{\scriptsize{(NP\_000676, NP\_005152)}}}
        \label{fig:diffa}
    \end{subfigure}%
    %
    \begin{subfigure}{0.26\textwidth}
        \centering
        \includegraphics[width=.9\textwidth]{figs/sim_matrix/P00748-NP_036559.jpg}
      	\caption{\mbox{\scriptsize{(P00748, NP\_036559)}}}
	\label{fig:diffb}
    \end{subfigure}
\\
\vspace{10pt}
    \begin{subfigure}{0.26\textwidth}
        \centering
        \includegraphics[width=.9\textwidth]{figs/sim_matrix/AAI28575-NP_066285.jpg}
       	\caption{\mbox{\scriptsize{(AAI28575, NP\_066285)}}}
	\label{fig:diffc}
    \end{subfigure}
    %
    \begin{subfigure}{0.26\textwidth}
        \centering
        \includegraphics[width=.9\textwidth]{figs/sim_matrix/AAB26273-NP_003605.jpg}
     	\caption{\mbox{\scriptsize{(AAB26273, NP\_003605)}}}
	\label{fig:diffd}
    \end{subfigure}
    \caption{Similarity matrices of target pairs with significant \rocauc improvement{/degradation}}
    \label{fig:perf_diff_similarity}
\end{figure*}


==> figs/supp_param_study_best_tasks_aada_dmpna_LG.tex <==
\begin{figure*}[h!]
    \centering
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/parameter_study/best_tasks_aada+dmpnna+L+G/mean-prc-auc.jpg}
        \caption{\prauc}
    \end{subfigure}
     ~ 
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/parameter_study/best_tasks_aada+dmpnna+L+G/mean-precision.jpg}
        \caption{\precision}
    \end{subfigure}
     ~
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/parameter_study/best_tasks_aada+dmpnna+L+G/mean-recall.jpg}
        \caption{\sensitivity}
    \end{subfigure}%
    
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/parameter_study/best_tasks_aada+dmpnna+L+G/mean-accuracy.jpg}
        \caption{\accuracy}
    \end{subfigure}
     ~ 
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/parameter_study/best_tasks_aada+dmpnna+L+G/mean-f1_score.jpg}
        \caption{\fone score}
    \end{subfigure}
    \caption{Parameter Study of \OurMethodWithDMPNNAWithDisc}
    \label{supp:fig:param_best_tasks_aada_dmpnna_LG}
\end{figure*}


==> tables/ablation.tex <==
\begin{table}[!h]
\centering
\caption{Comparison on Discriminators (with \newgnn)}
\label{tbl:ablation}
\begin{small}
  \begin{threeparttable}
      \begin{tabular}{
          @{\hspace{5pt}}l@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
    %      @{\hspace{5pt}}c@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
          }
          %
          \toprule
          method &  \rocauc & \prauc & \precision 
          & \sensitivity %& \tnr 
          & \accuracy & \fone \\
          \midrule
          \OurMethod & 0.801 & 0.786 & 0.731 & 0.729 & 0.720 & 0.713 \\
%		\midrule
%		\OurMethodWithDMPNNAWithDisc & 0.798 & 0.785 & 0.730 & 0.728 & 0.719 & 0.713 \\
%		\diff &  0.376 &  0.127 &  0.137 &  0.137 &  0.139 &  0.000 \\
%		\taskDiff &  0.404 &  0.166 &  0.215 &  1.260 &  0.230 &  0.503 \\
%		\pvalue &  2.59e-04 & 4.88e-01 & 7.26e-01 & 7.00e-01 & 5.53e-01 & 8.04e-01
%		\\
		\midrule
		 \OurMethodWithDisc & 0.798    & 0.785    & 0.730    & 0.728    & 0.719    & 0.713    \\
		 \cmidrule(lr){2-7}
		 \multicolumn{1}{r}{\diff}  & -0.375   & -0.127   & -0.137   & -0.137   & -0.139   & 0.000    \\
		 \multicolumn{1}{r}{\taskDiff}  & -0.380   & -0.119   & -0.072   & 0.116  & -0.150   & -0.064   \\
		 & (2.59e-04) & (4.88e-01) & (7.26e-01) & (7.00e-01)    & (5.53e-01) & (8.04e-01) \\
		 \multicolumn{1}{r}{\numImpv}  & 93 (39\%) & 125 (52\%) & 119 (50\%) & 111 (46\%) & 99 (41\%) & 112 (47\%)      \\
		 \multicolumn{1}{r}{\taskImpv} & 0.921    & 1.373    & 2.756    & 7.037    & 2.230    & 3.729    \\
		 & (7.73e-18) & (4.13e-23) & (1.69e-18) & (5.85e-19)  & (4.26e-14) & (1.31e-15)\\
	   %
	   %
	   \midrule
	   \OurMethodWithGlobalDisc & 0.801 & 0.786 & 0.730 & 0.734 &  0.721 & 0.716 \\
	   \cmidrule(lr){2-7}
%		\OurMethodWithDMPNNAWithDisc w/o \ldisc & 0.801 & 0.786 & 0.730 & 0.734 &  0.721 & 0.716 \\
		\multicolumn{1}{r}{\diff} & 0.000 & 0.000 & -0.137 & 0.686 & 0.139 & 0.421 \\
		 \multicolumn{1}{r}{\taskDiff} & 0.010 & -0.080 & -0.130 & 1.583 & 0.128 & 0.516 \\
		& (7.78e-01) & (6.72e-01) & (6.32e-01) & (3.03e-01) & (4.01e-01) & (3.90e-01) \\
		 \multicolumn{1}{r}{\numImpv} & 135 (56\%) & 119 (50\%) & 123 (51\%) & 126 (52\%) & 128 (53\%) & 130 (54\%) \\
		 \multicolumn{1}{r}{\taskImpv} & 0.845 & 1.330 & 2.763 & 8.798 & 1.971 & 4.165 \\
		& (1.13e-23) & (5.03e-24) & (2.67e-17) & (8.22e-18) &  (4.75e-21) & (1.75e-15) \\
		%
		%
		 \midrule
		\OurMethodWithLocalDisc  & 0.799 & 0.785 & 0.732 & 0.722 & 0.721 & 0.711 \\
		\cmidrule(lr){2-7}
%		\OurMethodWithDMPNNAWithDisc w/o \gdisc  & 0.799 & 0.785 & 0.732 & 0.722 & 0.721 & 0.711 \\
		\multicolumn{1}{r}{\diff} & -0.250 & -0.127 & 0.137 & -0.960 & 0.139 & -0.281 \\
		 \multicolumn{1}{r}{\taskDiff} & -0.192 & -0.091 & 0.218 & -0.768  & 0.170 & -0.326 \\
		& (4.00e-02) & (3.76e-01) & (5.44e-01) & (1.42e-01) & (3.19e-01) & (4.98e-01) \\
		 \multicolumn{1}{r}{\numImpv} & 100 (42\%) & 114 (48\%) & 124 (52\%) & 117 (49\%) & 125 (52\%) & 123 (51\%) \\
		 \multicolumn{1}{r}{\taskImpv} & 1.029 & 1.597 & 2.992 & 6.999 & 2.037 & 3.764 \\
		 & (3.22e-13) & (2.22e-21) & (3.85e-24) & (1.11e-19) & (9.65e-20) & (1.12e-16) \\
		 \bottomrule
		 \end{tabular}
		%
		
	\begin{tablenotes}
        \setlength\labelsep{0pt}
		\begin{footnotesize}
		\item In this table, 
		the first row block has the average performance of \OurMethod.
		Each of the other row blocks has performance comparison of a \OurMethodWithDisc
		variant with respect to \OurMethod.
		%
%		The rows \OurMethodWithDMPNNA, \OurMethodWithDMPNNAWithDisc,
%		\OurMethodWithDMPNNAWithDisc w/o \ldisc and
%		\OurMethodWithDMPNNAWithDisc w/o \gdisc
%		has the average performance in each evaluation metric from
%		respective methods.
		%
%		The row \diff in each row block has the percentage difference of average performance
%		in each metric
%		from the corresponding method in that row block over \OurMethodWithDMPNNA.
		The metric \diff represents the difference of average performance of each comparison 
		method with respect to \OurMethod;
		%
%		The row \taskDiff in each row block has the average of the task-wise percentage
%		improvement from the corresponding method over \OurMethodWithDMPNNA,
%		and the numbers in parentheses are their corresponding p-values.
		\taskDiff represents the average of the task-wise improvement, with corresponding $p$-values in the 
		parentheses below; 
		%
%		The row \numImpv has the number and percentage of improved tasks 
%		where the other method performs better 
%		than \OurMethodWithDMPNNA in respective metrics.
		\numImpv represents the number of improved tasks and its proportion in the parentheses; 
		%
%		The row \taskImpv has the average of task-wise percentage
%		improvement considering only corresponding \numImpv improved tasks,
%		and the numbers in parentheses are their corresponding p-values.
		and \taskImpv represents the average of the task-wise improvement only among the improved tasks, 
		with corresponding $p$-values in the parentheses below.
		\par
		\end{footnotesize}
	\end{tablenotes}

\end{threeparttable}
\end{small}
\end{table}

==> tables/best_perf_mean-roc-auc.tex <==
\begin{table}[h]
\centering
\caption{Overall Comparison}
\label{tbl:overall}
\begin{small}
  \begin{threeparttable}
      \begin{tabular}{
          @{\hspace{1pt}}l@{\hspace{1pt}}
          @{\hspace{1pt}}c@{\hspace{1pt}}
          @{\hspace{1pt}}c@{\hspace{1pt}}
          @{\hspace{1pt}}c@{\hspace{1pt}}
          @{\hspace{1pt}}c@{\hspace{1pt}}
    %      @{\hspace{1pt}}c@{\hspace{1pt}}
          @{\hspace{1pt}}c@{\hspace{1pt}}
          @{\hspace{1pt}}c@{\hspace{1pt}}
          }
          %
          \toprule
          method & \rocauc & \prauc & \precision 
          & \sensitivity %& \tnr 
          & \accuracy & \fone \\
          \midrule
          \morganFCN & 0.727$\pm$0.124 
          & 0.729$\pm$0.121 
          & 0.648$\pm$0.104 
          & \ul{0.742$\pm$0.131} 
          & 0.661$\pm$0.110 
          & \ul{0.683$\pm$0.105}
          \\
          \morgancFCN & 0.731$\pm$0.120 
          & 0.730$\pm$0.118 
          & 0.653$\pm$0.102 
          & 0.735$\pm$0.132 
          & 0.664$\pm$0.107 
          & 0.682$\pm$0.105
          \\
          \dmpnnFCN & 0.754$\pm$0.101 
          & 0.733$\pm$0.102 
          & 0.619$\pm$0.116 
          & 0.739$\pm$0.156 
          & 0.656$\pm$0.087 
          & 0.655$\pm$0.126
          \\
          \newgnnFCN & 0.755$\pm$0.112 
          & 0.729$\pm$0.112 
          & 0.660$\pm$0.119 
          & 0.712$\pm$0.165 
          & 0.665$\pm$0.101 
          & 0.651$\pm$0.136
          \\
          \dmpnnFCNDT & 0.754$\pm$0.104 
          & 0.735$\pm$0.105 
          & 0.687$\pm$0.106 
          & 0.686$\pm$0.213 
          & 0.669$\pm$0.088 
          & 0.655$\pm$0.140
          \\
          \newgnnFCNDT & \ul{0.763$\pm$0.108} 
          & \ul{0.745$\pm$0.109} 
          & \ul{0.702$\pm$0.108} 
          & 0.671$\pm$0.213 
          & \ul{0.672$\pm$0.092} 
          & 0.645$\pm$0.148
          \\
          \midrule
          \DANNWithDMPNN & 0.733$\pm$0.103
          & 0.715$\pm$0.103
          & 0.671$\pm$0.110
          & 0.647$\pm$0.215
          & 0.649$\pm$0.084
          & 0.623$\pm$0.144
          \\
          \DANNWithDMPNNA & 0.734$\pm$0.102
		 & 0.716$\pm$0.104
		 & 0.676$\pm$0.106
		 & 0.653$\pm$0.226
		 & 0.651$\pm$0.085
		 & 0.624$\pm$0.154
          \\
          \midrule
          \OurMethodWithDMPNN
          & 0.798$\pm$0.103 
          & 0.785$\pm$0.108 
          & 0.729$\pm$0.095 
          & 0.729$\pm$0.146 
          & \textbf{0.721$\pm$0.093}
          & 0.714$\pm$0.108
          \\
          \OurMethodWithDMPNNWithDisc & 0.798$\pm$0.102 
          & 0.784$\pm$0.107 
          & 0.729$\pm$0.094 
          & \textbf{0.731$\pm$0.142} 
          & 0.720$\pm$0.091 
          & \textbf{0.715$\pm$0.102}
          \\
          %\OurMethod\!\!\!+\dmpnn_combined & 0.802$\pm$0.102 & 0.788$\pm$0.107 & 0.732$\pm$0.096 & 0.731$\pm$0.144 & 0.715$\pm$0.140 & 0.723$\pm$0.092 & 0.716$\pm$0.105
          %\\
           \OurMethodWithDMPNNA 
           & \textbf{0.801$\pm$0.102} 
           & \textbf{0.786$\pm$0.107} 
           & \textbf{0.731$\pm$0.094} 
           & 0.729$\pm$0.143
           & 0.720$\pm$0.090
           & 0.713$\pm$0.103
          \\
          \OurMethodWithDMPNNAWithDisc & 0.798$\pm$0.105 
          & 0.785$\pm$0.109 
          & 0.730$\pm$0.097 
          & 0.728$\pm$0.147 
          & 0.719$\pm$0.095 
          & 0.713$\pm$0.109
          \\
           %\OurMethod\!\!\!+\newgnn_combined & 0.804$\pm$0.102 & 0.790$\pm$0.106 & 0.734$\pm$0.096 & 0.732$\pm$0.143 & 0.714$\pm$0.140 & 0.723$\pm$0.093 & 0.717$\pm$0.105
%          \midrule
%          \newgnnFCNDT & 0.763$\pm$0.108 
%           & 0.745$\pm$0.109 
%           & 0.702$\pm$0.108 
%           & 0.671$\pm$0.213 
%           & 0.672$\pm$0.092 
%           & 0.645$\pm$0.148
%          \\
%          \diff &  4.980 & 5.503 & 4.131 & 8.644 & 7.143 & 10.543
%	 \\
%	 \taskDiff & 5.702 & 6.085 & 4.876 & 25.281 & 7.727 & 18.464
%	\\
%	\pvalue & 2.80e-19 & 8.00e-21 & 1.69e-11 & 1.73e-09 & 1.19e-29 & 8.93e-20
%	 \\
%	 \numImpv  & 199 (83\%) & 192 (80\%) & 157 (65\%) & 153 (64\%) & 201 (84\%) & 198 (82\%)  \\
%	 \taskImpv &  7.102 &  8.044 &  9.293 &  44.261 &  9.509 &  23.532 \\
%	 \pvalue &  5.56e-22 &  5.51e-26 &  2.81e-27 &  7.36e-25 &  5.02e-35 &  3.60e-26
%	 \\
	\bottomrule
	\end{tabular}
	%

	\begin{tablenotes}
        \setlength\labelsep{0pt}
		\begin{footnotesize}
		\item In this table, the columns \rocauc, \prauc, \precision, \sensitivity, %specificity\vmodified{TNR}.
		\accuracy and \fone-score 
		have the average and standard deviation 
		over all bioassays in each performance metric.
		%
		The best performance values are \textbf{boldfaced}. The second best performance values are \ul{underlined}.
		%
%		The row \diff has the percentage difference of average \OurMethodWithDMPNNA performance
%		over average \newgnnFCNDT performance in respective metrics.
%		%
%		The row \taskDiff has the average of task-wise percentage
%		improvement from \OurMethodWithDMPNNA over
%		\newgnnFCNDT in respective metrics.
%		%
%		The row \numImpv has the number and percentage of target tasks where \OurMethodWithDMPNNA
%		performs better than \newgnnFCNDT in respective metrics.
%		%
%		The row \taskImpv has the average of task-wise percentage
%		improvement considering only corresponding \numImpv improved tasks.
%		The row \pvalue has the p-values for corresponding \taskDiff/\taskImpv.
		\par
		\end{footnotesize}
	\end{tablenotes}

\end{threeparttable}
\end{small}
\end{table}

==> tables/best_ranking.tex <==
\begin{table}[h]
\sisetup{input-decimal-markers={.}, round-mode=places, round-precision=3}  
\centering
\caption{Overall Performance Comparison of \RankMethod} 
\label{tbl:best_ranking}
\begin{small}
  \begin{threeparttable}
      \begin{tabular}{
          @{\hspace{5pt}}l@{\hspace{5pt}}
          %
          @{\hspace{5pt}}r@{\hspace{5pt}}
          %
          @{\hspace{5pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
          %@{\hspace{5pt}}r@{\hspace{5pt}}
          % 
          @{\hspace{5pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
         % @{\hspace{5pt}}r@{\hspace{5pt}}
          %
          @{\hspace{5pt}}r@{\hspace{5pt}}
          %@{\hspace{5pt}}r@{\hspace{5pt}}
          %
          @{\hspace{5pt}}r@{\hspace{5pt}} 
         % @{\hspace{5pt}}r@{\hspace{5pt}}
          }
          \toprule
          method & CI & 
          R\text{@3} & R\text{@5} & %R\text{@10} &
          ndcg\text{@3} & ndcg\text{@5} & %ndcg\text{@10} & 
          R\text{@5\%} & %R\text{@10\%} &
          \small{ndcg\text{@5\%}} %& \small{ndcg\text{@10\%}} 
          \\
          \midrule
			%
			\MORGAN & 0.706 & 0.543 & 0.644 %& 0.853 
			& 0.814 & 0.816 %& 0.871 
			& 0.420 %& 0.477 
			& 0.838 %& 0.819
			\\
			\MORGANC & 0.711 & 0.545 & 0.655 %& 0.855 
			& 0.815 & 0.819 %& 0.872 
			& 0.437 %& 0.487 
			& 0.846 %& 0.822 
			\\
			\MORGANBA & 0.687 & 0.500 & 0.626 %& 0.844 
			& 0.789 & 0.797 %& 0.857 
			& 0.375 %& 0.436 
			& 0.816 %& 0.800
			\\
			\RDKITGD & 0.687 & 0.519 & 0.632 %& 0.839 
			& 0.790 & 0.797 %& 0.853 
			& 0.396 %& 0.461 
			& 0.813 %& 0.796 
			\\
			\dmpnn & \underline{0.731} & \underline{0.643} & \underline{0.709} %& \underline{0.879}  
			& \underline{0.854} & \underline{0.847} %& \underline{0.887}
			& \underline{0.579} %& \underline{0.599} 
			& \underline{0.896} %& \underline{0.866} 
			\\
			\midrule
			\newgnn & \textbf{0.748} & \textbf{0.686} & \textbf{0.740} %& \textbf{0.891} 
			& \textbf{0.881} & \textbf{0.867} %& \textbf{0.900}
			& \textbf{0.686} %& \textbf{0.666} 
			& \textbf{0.936} %& \textbf{0.900}
			\\			
			\diff & 2.353 & 6.608 & 4.460 %& 1.388
			& 3.114 & 2.421 %& 1.454
			& 18.428 %& 11.154
			& 4.475 %& 3.878 
			\\
			\taskDiff & 2.535 & 7.645 & 4.720 %& 1.460 
			& 3.406 & 2.569 %& 1.527
			& 24.578 %& 13.399 
			& 4.979 %& 4.245 
			\\
			\pvalue & 1.14e-10 & 4.89e-10 & 9.87e-13 %& 8.56e-10 
			& 1.42e-12 & 2.25e-12 %& 5.3e-09
			& 3.95e-15 %& 1.74e-14 
			& 1.83e-11 %& 2.11e-12 
			\\
 		\bottomrule
		\end{tabular}
		%
		\begin{tablenotes}
        \setlength\labelsep{0pt}
		\begin{footnotesize}
		%
		\item
		In this table, the columns have the respective average of each performance metric 
		over all bioassays obtained by the 	
		respective optimal hyperparameter settings.
		The best/second best performance under each metric is \textbf{bold}/\underline{underlined}. 
%		The second best performance  is \underline{underlined}. % are obtained by {\dmpnn}. %Among the baselines, the best performance values (italicized) are obtained from the \MORGANC baseline.
		\end{footnotesize}
		\end{tablenotes}
\end{threeparttable}
\end{small}
\end{table}


==> tables/defs.tex <==
\begin{table}
\centering
\caption{Notations}
\label{tbl:defs}
\begin{small}
  \begin{threeparttable}
      \begin{tabular}{
          @{\hspace{3pt}}l@{\hspace{3pt}}
          @{\hspace{3pt}}l@{\hspace{3pt}}
          }
          \toprule
          notations & meanings \\
          \midrule
          %
          \compound/\bioassay & compound/bioassay \\
          \MolGraph = (\SetAtoms, \SetBonds) & molecular graph with set of 
          atoms \SetAtoms and bonds \SetBonds  \\
%          $n$ & number of compounds in a bioassay \\
%          $n_a$ & number of active compounds in a bioassay \\
%          $n_i$ & number of inactive compounds in a bioassay \\
          %
          $u$ & an atom in \MolGraph \\
          $(u, v)$ & a bond connecting atoms $u$ and $v$ in \MolGraph \\
          $\mathcal{N}(u)$ & neighbors of atom $u$ in \MolGraph \\
%          $\AtomFeature_{u}$ & initial feature vector of an atom $u$ \\
%          $\BondFeature_{uv}$ & initial feature vector of a bond $(u, v)$ \\
%          $\InputFeature = (\AtomFeature, \BondFeature)$ & 
%          input feature of a compound consisting of initial atom and edge features \\
%          $\tau$ & number of message-passing steps \\
%          $\mes_{uv}^{(t)}$ & aggregated message over bond $(u, v)$ at step $t$ \\
%       	\hidden & hidden state \\  	  
          %
          \SetCompounds & set of compounds in a bioassay \\
          \SetLabels & set of labels corresponding to \SetCompounds \\
          \FeatureSpace & input feature space \\
          \LabelSpace & label space \\
          $\domain = \{\FeatureSpace, P(\SetCompounds)\}$ & a domain consisting of
          \FeatureSpace and marginal probability distribution P(\SetCompounds) \\
          $\task = \{\LabelSpace, \omega(\cdot)\}$ & a task consisting of label space and a 
          decision function $\omega(\cdot)$  \\
          %
%          \fgnn & feature extractor implemented using \gnn  \\
%          \ldisc & local discriminator \\
%          \gdisc & global discriminator \\
%          \classifier & classifier of the model \\
%          $\fatt_{\cdot}$ & attention-based pooling function in \newgnn \\
%          \FinalLoss & final loss function \\
%          \LocalDiscLoss & local discriminator loss function \\
%       	  \GlobalDiscLoss & global discriminator loss function \\
%       	  \ClassifierLoss & classification loss function \\
%     %  	 $\lambda$ & trade-off parameter \\
%       	 %
%       	 \prob & probability vector out of \ldisc \\
%       	 $\chi(\cdot)$ & feature scaling function \\
%       	 %
%       	 \entropy & Entropy \\
%       	 $\mathbb{E}$ & Expectation \\
		 \hidden & hidden state \\
       	  \compr & molecular representation out of \gnn \\
       	  \scompr & scaled molecular representation \\
%       	 $d$ & dimension of \compr, \ModifiedCompr, \prob \\
%       	 \params & model trainable parameters \\
          \bottomrule
          \end{tabular}
		%
		%
\end{threeparttable}
\end{small}
\end{table}


==> tables/parameters.tex <==
\begin{table}[h]
\centering
\caption{Hyperparameter Configurations}
\label{tbl:supp:parameters}
  \begin{threeparttable}
      \begin{tabular}{
          @{\hspace{5pt}}l@{\hspace{5pt}}
          @{\hspace{5pt}}c@{\hspace{5pt}}
          }
          %
          \toprule
          parameter & values \\
          \midrule
          $\alpha$ & {0, 0.1, 0.5, 1, 2} \\
          $\lambda$ & {0.001, 0.01, 0.5, 1} \\
          dimension $d$ & {25, 50, 100} \\
          \# message passing steps $\tau$   &    {2, 3, 4} \\
          hidden layer size in $\fatt(\cdot)$	& 		{100} \\
		 hidden layer size in $\ldisc$, $\gdisc$ and $\classifier$  &   {100} \\
          batch size   	& 	{10} \\
          learning rate & {1e-3} \\
          \bottomrule
		 \end{tabular}
		%
%		\begin{tablenotes}
%        \setlength\labelsep{0pt}
%		\begin{footnotesize}
%		\item In this table, the different values of hyper-parameters for the baselines and proposed methods
%		are presented.
%		\end{footnotesize}
%		\end{tablenotes}
%	
	
\end{threeparttable}
\end{table}

==> tables/perf_imp_best_2ndbest.tex <==
\begin{table}[h]
\centering
\caption{Performance Comparison of \OurMethodWithDMPNNA vs \newgnnFCN}
\label{tbl:perf_imp_best}

\begin{threeparttable}
	\begin{tabular}{
		@{\hspace{2pt}}l@{\hspace{2pt}}
		@{\hspace{2pt}}c@{\hspace{2pt}}
		@{\hspace{2pt}}c@{\hspace{2pt}}
		@{\hspace{2pt}}c@{\hspace{2pt}}
		@{\hspace{2pt}}c@{\hspace{2pt}}
%      @{\hspace{2pt}}c@{\hspace{2pt}}
		@{\hspace{2pt}}c@{\hspace{2pt}}
       	@{\hspace{2pt}}c@{\hspace{2pt}}
      	}
      	%
        \toprule
        	method & \rocauc & \prauc & \precision 
      	& \sensitivity %& \tnr 
      	& \accuracy & \fone \\
     	\midrule
         \OurMethodWithDMPNNA 
       	& 0.801  & 0.786   & 0.731
       	& 0.729  & 0.720   & 0.713
      	\\
      	\newgnnFCNDT 
      	& 0.763  & 0.745  & 0.702  
        	& 0.671  & 0.672  & 0.645
 		\\
       	\diff & 4.980 & 5.503 & 4.131 & 8.644 & 7.143 & 10.543
      	\\
      	\multirow{2}{*}{\taskDiff} & 5.702 & 6.085 & 4.876 
      	& 25.281  & 7.727 & 18.464
       	\\
        	 & (2.80e-19) & (8.00e-21) & (1.69e-11) & (1.73e-09) & (1.19e-29) & (8.93e-20)
        	\\
        	\numImpv  & 199 (83\%) & 192 (80\%) & 157 (65\%) & 153 (64\%) & 201 (84\%) & 198 (82\%)  
        	\\
        	\multirow{2}{*}{\taskImpv} &  7.102 &  8.044 &  9.293 &  44.261 &  9.509 &  23.532 
        	\\
 		 &  (5.56e-22) &  (5.51e-26) & (2.81e-27) & (7.36e-25) & (5.02e-35) & (3.60e-26)
 		\\
 		\bottomrule
	\end{tabular}
 	
	\begin{tablenotes}
        \setlength\labelsep{0pt}
		\begin{footnotesize}
		\item In this table, the first two rows
		has the	performance from respective methods averaged
		over all bioassays in each performance metric.
		%
%		The row \diff has the percentage difference of average \OurMethodWithDMPNNA performance
%		over average \newgnnFCNDT performance in respective metrics.
		The row \diff has the percentage difference of average performance in 
		each metric from \OurMethodWithDMPNNA
		over \newgnnFCNDT.
		%
		The row \taskDiff has the average of task-wise percentage
		improvement from \OurMethodWithDMPNNA over
		\newgnnFCNDT in respective metrics, with corresponding p-value in parentheses below.
		%
		The row \numImpv has the number and percentage of target tasks where \OurMethodWithDMPNNA
		performs better than \newgnnFCNDT in respective metrics.
		%
		The row \taskImpv has the average of task-wise percentage
		improvement only among the corresponding improved tasks,
		with corresponding pvalues in parentheses below.
		\par
		\end{footnotesize}
	\end{tablenotes}

\end{threeparttable}
\end{table}

==> tables/supp_TP_pred_analysis_Tac-c_vs_variants.tex <==
\begin{ThreePartTable}
\centering
\begin{TableNotes}
\item In this table, the columns source(S) and target(T) correspond to 
the protein accession numbers of the corresponding bioassays of source and target tasks, respectively. 
The columns \#cor, \#act and cor\%
have the count of correctly classified active compounds,
total number of active compounds and 
the percentage of correctly classified active compounds, respectively.
Such compounds are denoted by the set $\tilde{\SetCompounds}_{\scriptsize \bioassay_T}^{+}$.
The columns
$\text{sim}(\tilde{\SetCompounds}_{\scriptsize \bioassay_T}^{+}, \SetCompounds_{\scriptsize \bioassay_S}^{+})$ and
$\text{sim}(\tilde{\SetCompounds}_{\scriptsize \bioassay_T}^{+}, \SetCompounds_{\scriptsize \bioassay_T}^{+})$
present the average pairwise similarities 
of correctly classified compounds in $\tilde{\SetCompounds}_{\scriptsize \bioassay_T}^{+}$ 
with their top-5 most similar active compounds 
from the source and target bioassay, respectively.
The column \simDiff has the percentage difference of the 
average pairwise similarities from the source compounds
over the target compounds.
The column \eSimDiff has the average of element-wise percentage difference
of similarities from the source active compounds over the target active compounds.
The column \pvalue has the corresponding p-values for \eSimDiff.
\par
\end{TableNotes}

\begin{small}
\begin{longtable}[h]
		{
		 @{\hspace{1pt}}c@{\hspace{1pt}}
         @{\hspace{1pt}}c@{\hspace{0pt}}
         @{\hspace{0pt}}r@{\hspace{1pt}}
         @{\hspace{1pt}}r@{\hspace{1pt}}
         @{\hspace{1pt}}r@{\hspace{1pt}}
         @{\hspace{1pt}}r@{\hspace{1pt}}
         @{\hspace{1pt}}r@{\hspace{1pt}}
         @{\hspace{1pt}}r@{\hspace{1pt}}
         @{\hspace{1pt}}r@{\hspace{1pt}}
         @{\hspace{1pt}}r@{\hspace{1pt}}
         }
          %
        \caption{Similarity analysis of correct predictions by \OurMethodWithGlobalDisc}
		\label{tbl:supp:TP_preds_analysis_TAc-c} \\
		%
		\midrule
        	source(S)  &  target(T) & \#cor & \#act & cor\% &
        \footnotesize{$\text{sim}(\tilde{\SetCompounds}_{\tiny \bioassay_T}^{+}, \SetCompounds_{\tiny \bioassay_S}^{+})$}
        & \footnotesize{$\text{sim}(\tilde{\SetCompounds}_{\tiny \bioassay_T}^{+}, \SetCompounds_{\tiny \bioassay_T}^{+})$}
        	& \simDiff & \eSimDiff & \pvalue \\
        \midrule
        \endfirsthead
        %
        \multicolumn{10}{c}%
        {{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
		%
		\midrule
        source(S)  &  target(T) & \#cor & \#act & cor\% &
        \footnotesize{$\text{sim}(\tilde{\SetCompounds}_{\tiny \bioassay_T}^{+}, \SetCompounds_{\tiny \bioassay_S}^{+})$}
        & \footnotesize{$\text{sim}(\tilde{\SetCompounds}_{\tiny \bioassay_T}^{+}, \SetCompounds_{\tiny \bioassay_T}^{+})$}
        	& \simDiff & \eSimDiff & \pvalue \\
        \midrule
        \endhead
        %
        \midrule
        \multicolumn{10}{|r|}{{Continued on next page}} \\
        \endfoot
        %
        \midrule
        \insertTableNotes
        \endlastfoot
		%
EAW86722 & AAI27629 & 36 & 128 & 28.125 & 0.231 & 0.194 & 19.401 & 21.692 & 1.68e-05 \\
NP\_004818 & ABD72211 & 131 & 485 & 27.010 & 0.191 & 0.218 & -12.557 & -12.312 & 3.05e-20 \\
NP\_000901 & NP\_001516 & 33 & 124 & 26.613 & 0.213 & 0.182 & 17.135 & 19.886 & 2.57e-05 \\
NP\_000483 & NP\_000918 & 18 & 82 & 21.951 & 0.262 & 0.444 & -41.090 & -32.693 & 1.56e-05 \\
NP\_004942 & NP\_003605 & 29 & 145 & 20.000 & 0.164 & 0.174 & -5.916 & -2.832 & 4.15e-01 \\
NP\_004221 & NP\_001516 & 21 & 124 & 16.935 & 0.212 & 0.203 & 4.530 & 6.081 & 2.45e-01 \\
AAC63054 & AAF04852 & 85 & 546 & 15.568 & 0.255 & 0.249 & 2.490 & 3.969 & 1.25e-01 \\
NP\_001516 & NP\_000947 & 15 & 112 & 13.393 & 0.244 & 0.193 & 26.449 & 28.965 & 2.92e-04 \\
EAW86722 & NP\_004358 & 6 & 46 & 13.043 & 0.239 & 0.144 & 66.156 & 66.256 & 5.06e-06 \\
AAH04460 & AAH14460 & 6 & 55 & 10.909 & 0.228 & 0.154 & 47.925 & 50.102 & 2.68e-05 \\
P00748 & NP\_004521 & 8 & 85 & 9.412 & 0.227 & 0.209 & 8.621 & 11.614 & 2.38e-01 \\
P00748 & AAF04852 & 50 & 546 & 9.158 & 0.237 & 0.267 & -11.053 & -8.667 & 1.22e-04 \\
P00748 & NP\_660205 & 57 & 634 & 8.991 & 0.243 & 0.242 & 0.662 & 1.593 & 6.55e-01 \\
NP\_004942 & NP\_000676 & 15 & 168 & 8.929 & 0.183 & 0.216 & -15.296 & -11.831 & 8.28e-03 \\
EAW86722 & NP\_000947 & 10 & 112 & 8.929 & 0.240 & 0.208 & 15.663 & 17.138 & 1.41e-01 \\
AAC63054 & AAI29989 & 55 & 638 & 8.621 & 0.234 & 0.249 & -6.064 & -3.701 & 1.69e-02 \\
NP\_001391 & NP\_001516 & 10 & 123 & 8.130 & 0.269 & 0.201 & 33.649 & 34.022 & 1.13e-06 \\
EAW86722 & AAH14970 & 8 & 99 & 8.081 & 0.266 & 0.212 & 25.838 & 28.634 & 1.58e-02 \\
AAI29989 & AAF04852 & 22 & 273 & 8.059 & 0.315 & 0.213 & 48.214 & 50.797 & 3.80e-10 \\
NP\_036559 & AAI29989 & 51 & 636 & 8.019 & 0.244 & 0.258 & -5.124 & -4.478 & 5.37e-03 \\
BAB91222 & AAH14970 & 8 & 101 & 7.921 & 0.175 & 0.165 & 5.943 & 8.653 & 3.60e-01 \\
P00748 & NP\_036559 & 5 & 67 & 7.463 & 0.271 & 0.184 & 47.440 & 43.716 & 8.58e-02 \\
NP\_004358 & AAH14970 & 7 & 98 & 7.143 & 0.207 & 0.167 & 24.161 & 23.704 & 9.37e-03 \\
AAA51985 & NP\_036559 & 5 & 70 & 7.143 & 0.226 & 0.167 & 35.308 & 35.516 & 1.30e-03 \\
BAB91222 & NP\_000901 & 5 & 71 & 7.042 & 0.252 & 0.166 & 51.322 & 52.216 & 2.77e-02 \\
NP\_004358 & NP\_001516 & 8 & 124 & 6.452 & 0.195 & 0.196 & -0.357 & 2.666 & 9.42e-01 \\
AAH14460 & AAC63054 & 11 & 176 & 6.250 & 0.240 & 0.237 & 1.395 & 4.762 & 8.31e-01 \\
NP\_003984 & EAW70217 & 7 & 112 & 6.250 & 0.176 & 0.207 & -15.381 & -10.736 & 2.51e-01 \\
NP\_001516 & NP\_000676 & 10 & 168 & 5.952 & 0.215 & 0.177 & 21.813 & 25.027 & 4.71e-02 \\
NP\_000900 & NP\_001391 & 16 & 273 & 5.861 & 0.207 & 0.187 & 10.512 & 13.962 & 5.45e-02 \\
EAW86722 & NP\_000901 & 4 & 70 & 5.714 & 0.211 & 0.153 & 37.288 & 39.267 & 3.66e-04 \\
NP\_004062 & NP\_005424 & 16 & 294 & 5.442 & 0.178 & 0.191 & -6.695 & -4.963 & 1.83e-01 \\
NP\_001516 & AAB26273 & 12 & 222 & 5.405 & 0.192 & 0.173 & 11.478 & 13.326 & 2.22e-02 \\
AAH14460 & P00748 & 6 & 118 & 5.085 & 0.209 & 0.176 & 19.259 & 19.193 & 9.09e-03 \\
ADZ17337 & NP\_000448 & 6 & 119 & 5.042 & 0.216 & 0.378 & -42.872 & -26.487 & 7.48e-02 \\
EAW86722 & AAB26273 & 11 & 222 & 4.955 & 0.171 & 0.172 & -0.639 & -0.201 & 9.25e-01 \\
AAB26273 & AAH14970 & 5 & 101 & 4.950 & 0.237 & 0.191 & 23.628 & 30.287 & 1.59e-01 \\
AAI28575 & ADZ17337 & 3 & 62 & 4.839 & 0.195 & 0.122 & 59.508 & 59.696 & 6.99e-03 \\
NP\_004358 & AAB26273 & 10 & 222 & 4.505 & 0.180 & 0.181 & -0.222 & 1.167 & 9.65e-01 \\
P00748 & NP\_004337 & 27 & 623 & 4.334 & 0.244 & 0.271 & -9.934 & -7.917 & 2.86e-03 \\
AAB26273 & NP\_000901 & 3 & 70 & 4.286 & 0.200 & 0.158 & 26.692 & 33.966 & 1.20e-01 \\
AAB26273 & NP\_000676 & 7 & 167 & 4.192 & 0.217 & 0.294 & -26.226 & -17.244 & 1.02e-01 \\
AAA51985 & P00748 & 4 & 98 & 4.082 & 0.254 & 0.185 & 37.324 & 38.576 & 3.26e-02 \\
AAA51985 & AAI29989 & 26 & 639 & 4.069 & 0.227 & 0.243 & -6.579 & -5.651 & 1.71e-02 \\
AAB26273 & EAW86722 & 11 & 280 & 3.929 & 0.253 & 0.359 & -29.579 & -7.283 & 1.26e-01 \\
NP\_036559 & AAF04852 & 21 & 545 & 3.853 & 0.224 & 0.237 & -5.495 & -3.310 & 2.10e-01 \\
AAH14460 & AAH04460 & 13 & 356 & 3.652 & 0.154 & 0.136 & 12.702 & 12.870 & 1.06e-04 \\
NP\_004358 & NP\_000900 & 3 & 83 & 3.614 & 0.211 & 0.181 & 16.860 & 15.934 & 1.37e-01 \\
NP\_000901 & EAW86722 & 10 & 280 & 3.571 & 0.251 & 0.503 & -50.099 & -46.770 & 1.25e-04 \\
NP\_004818 & NP\_000483 & 5 & 143 & 3.497 & 0.205 & 0.190 & 8.065 & 8.009 & 1.57e-01 \\
AAF04852 & AAC63054 & 6 & 179 & 3.352 & 0.318 & 0.215 & 48.069 & 49.310 & 5.66e-04 \\
AAI29989 & NP\_660205 & 12 & 395 & 3.038 & 0.287 & 0.191 & 49.869 & 52.166 & 3.98e-05 \\
NP\_775180 & ADZ17337 & 2 & 67 & 2.985 & 0.181 & 0.143 & 26.606 & 25.601 & 2.58e-01 \\
NP\_000448 & ADZ17337 & 2 & 68 & 2.941 & 0.114 & 0.060 & 91.779 & 95.379 & 7.93e-02 \\
ADZ17337 & NP\_066285 & 4 & 137 & 2.920 & 0.221 & 0.204 & 8.640 & 10.717 & 2.39e-01 \\
AAC63054 & NP\_004337 & 18 & 623 & 2.889 & 0.264 & 0.271 & -2.731 & 0.234 & 5.85e-01 \\
NP\_004358 & NP\_000901 & 2 & 71 & 2.817 & 0.154 & 0.123 & 25.345 & 26.218 & 3.06e-01 \\
AAF04852 & NP\_004337 & 8 & 287 & 2.787 & 0.321 & 0.218 & 47.407 & 50.401 & 6.15e-03 \\
AAB26273 & NP\_000947 & 3 & 108 & 2.778 & 0.232 & 0.158 & 46.717 & 52.124 & 7.21e-02 \\
AAB26273 & NP\_003605 & 4 & 144 & 2.778 & 0.219 & 0.151 & 44.746 & 43.328 & 3.17e-02 \\
NP\_000901 & BAB91222 & 2 & 73 & 2.740 & 0.266 & 0.584 & -54.493 & -54.476 & 2.78e-02 \\
AAH14970 & AAB26273 & 6 & 222 & 2.703 & 0.191 & 0.164 & 16.190 & 16.216 & 7.96e-02 \\
BAB91222 & AAB26273 & 6 & 222 & 2.703 & 0.160 & 0.167 & -4.540 & -3.455 & 2.74e-01 \\
BAB91222 & NP\_000947 & 3 & 112 & 2.679 & 0.206 & 0.214 & -3.745 & -2.894 & 7.53e-01 \\
P00748 & AAC63054 & 4 & 153 & 2.614 & 0.259 & 0.249 & 3.974 & 5.017 & 7.69e-01 \\
BAB91222 & NP\_001391 & 7 & 276 & 2.536 & 0.158 & 0.183 & -13.803 & -13.149 & 1.29e-02 \\
%NP\_000448 & AAI28575 & 6 & 243 & 2.469 & 0.101 & 0.094 & 7.234 & 32.271 & 2.57e-01 \\
AAH14460 & NP\_036559 & 2 & 81 & 2.469 & 0.246 & 0.186 & 32.453 & 32.468 & 6.44e-02 \\
NP\_004337 & P00748 & 3 & 128 & 2.344 & 0.270 & 0.191 & 41.575 & 43.957 & 1.01e-02 \\
AAI29989 & NP\_036559 & 2 & 87 & 2.299 & 0.227 & 0.150 & 52.107 & 51.804 & 3.36e-01 \\
NP\_004337 & AAC63054 & 4 & 179 & 2.235 & 0.283 & 0.197 & 43.357 & 42.784 & 4.74e-03 \\
NP\_000760 & NP\_000752 & 17 & 828 & 2.053 & 0.265 & 0.197 & 34.518 & 40.100 & 4.00e-05 \\
AAA51985 & AAC63054 & 3 & 160 & 1.875 & 0.263 & 0.212 & 24.034 & 24.481 & 8.67e-03 \\
NP\_000903 & EAW86722 & 5 & 267 & 1.873 & 0.236 & 0.507 & -53.336 & -52.539 & 1.96e-03 \\
NP\_000900 & AAB26273 & 4 & 222 & 1.802 & 0.192 & 0.172 & 11.874 & 21.471 & 5.88e-01 \\
NP\_612200 & AAB26273 & 4 & 222 & 1.802 & 0.205 & 0.192 & 7.035 & 12.079 & 6.27e-01 \\
NP\_004705 & EAW70217 & 2 & 112 & 1.786 & 0.176 & 0.153 & 15.465 & 15.582 & 3.20e-03 \\
AAI29989 & AAC63054 & 3 & 179 & 1.676 & 0.275 & 0.195 & 40.963 & 43.788 & 1.15e-01 \\
EAW86722 & NP\_000903 & 2 & 121 & 1.653 & 0.201 & 0.119 & 68.483 & 73.823 & 1.13e-02 \\
BAH02301 & AAI28575 & 4 & 243 & 1.646 & 0.199 & 0.155 & 28.479 & 30.254 & 2.86e-02 \\
AAI29989 & P00748 & 2 & 128 & 1.563 & 0.307 & 0.187 & 63.821 & 68.477 & 2.76e-01 \\
NP\_660205 & P00748 & 2 & 128 & 1.563 & 0.223 & 0.199 & 12.042 & 18.287 & 3.47e-01 \\
NP\_000762 & NP\_000752 & 11 & 768 & 1.432 & 0.252 & 0.223 & 12.713 & 16.400 & 7.20e-02 \\
BAB91222 & EAW86722 & 4 & 280 & 1.429 & 0.212 & 0.395 & -46.403 & -45.265 & 1.19e-02 \\
NP\_000918 & NP\_000483 & 2 & 143 & 1.399 & 0.181 & 0.167 & 8.313 & 8.153 & 2.06e-01 \\
NP\_066285 & AAI28575 & 3 & 244 & 1.230 & 0.224 & 0.175 & 28.138 & 28.295 & 3.79e-02 \\
P00748 & AAI29989 & 7 & 638 & 1.097 & 0.234 & 0.325 & -27.930 & -17.446 & 1.11e-01 \\
AAB26273 & NP\_001391 & 3 & 274 & 1.095 & 0.236 & 0.220 & 7.039 & 8.095 & 7.11e-01 \\
NP\_004942 & NP\_997055 & 19 & 2,020 & 0.941 & 0.174 & 0.233 & -25.354 & -24.636 & 1.43e-07 \\
NP\_002721 & NP\_001387 & 2 & 216 & 0.926 & 0.157 & 0.262 & -40.099 & -15.747 & 5.69e-01 \\
NP\_001387 & NP\_065717 & 3 & 411 & 0.730 & 0.303 & 0.358 & -15.284 & -11.201 & 3.77e-01 \\
AAF04852 & AAI29989 & 2 & 278 & 0.719 & 0.233 & 0.190 & 22.866 & 23.111 & 5.88e-02 \\
NP\_000947 & EAW86722 & 2 & 280 & 0.714 & 0.219 & 0.166 & 31.671 & 31.738 & 6.30e-04 \\
NP\_004337 & AAI29989 & 2 & 303 & 0.660 & 0.272 & 0.211 & 28.856 & 28.826 & 6.91e-02 \\
NP\_004705 & NP\_005021 & 50 & 8,158 & 0.613 & 0.163 & 0.249 & -34.671 & -33.500 & 5.32e-14 \\
NP\_000752 & NP\_000760 & 3 & 543 & 0.552 & 0.299 & 0.247 & 21.330 & 23.816 & 3.93e-01 \\
NP\_036559 & NP\_004337 & 2 & 622 & 0.322 & 0.252 & 0.246 & 2.153 & 3.971 & 8.75e-01 \\
NP\_002825 & NP\_004081 & 2 & 1,316 & 0.152 & 0.261 & 0.254 & 2.678 & 2.762 & 8.02e-03
\end{longtable}
\end{small}
\end{ThreePartTable}

==> tables/supp_bioassay_pairs_stat.tex <==
\begin{ThreePartTable}
\centering
\begin{TableNotes}
\item In this table, the first two columns target(P) and target(Q) 
correspond to the accession numbers of the two target proteins 
corresponding to the two bioassays P and Q of the pair, respectively.
The columns 
$|\SetCompounds_{\scriptsize \bioassay_A}|$ %($|\SetCompounds_{\scriptsize \bioassay_Q}|$),
$|\SetCompounds_{\scriptsize \bioassay_A}^{+}|$ %($|\SetCompounds_{\scriptsize \bioassay_Q}^{+}|$)
and $|\SetCompounds_{\scriptsize \bioassay_A}^{-}|$ %($|\SetCompounds_{\scriptsize \bioassay_Q}^{-}|$)
correspond to the number of
total compounds, active compounds and inactive compounds in the bioassay $A$  
where ($A = \{P, Q\}$ of each pair).
\par
\end{TableNotes}


\begin{longtable}[h]
	{
      	  @{\hspace{8pt}}r@{\hspace{8pt}}
          @{\hspace{8pt}}r@{\hspace{8pt}}
          @{\hspace{8pt}}r@{\hspace{8pt}}
          @{\hspace{8pt}}r@{\hspace{8pt}}
          @{\hspace{8pt}}r@{\hspace{8pt}}
          @{\hspace{8pt}}r@{\hspace{8pt}}
          @{\hspace{8pt}}r@{\hspace{8pt}}
          @{\hspace{8pt}}r@{\hspace{8pt}}
        }

	\caption{Compound statistics of selected bioassay pairs}
	\label{tbl:supp:pairs_stat} \\
	%
	\midrule
        	target(P) & target(Q) & $|\SetCompounds_{\scriptsize \bioassay_P}|$
        	& $|\SetCompounds_{\scriptsize \bioassay_P}^{+}|$ 
        	& $|\SetCompounds_{\scriptsize \bioassay_P}^{-}|$
        %& |\#total-B & \#active-B & \#inactive-B
        & $|\SetCompounds_{\scriptsize \bioassay_Q}|$
        	& $|\SetCompounds_{\scriptsize \bioassay_Q}^{+}|$ 
        	& $|\SetCompounds_{\scriptsize \bioassay_Q}^{-}|$
        \\ 
        \midrule
        \endfirsthead
        %
        
        \multicolumn{8}{c}%
        {{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
	%
	\midrule
        	target(P) & target(Q) & $|\SetCompounds_{\scriptsize \bioassay_P}|$
        	& $|\SetCompounds_{\scriptsize \bioassay_P}^{+}|$ 
        	& $|\SetCompounds_{\scriptsize \bioassay_P}^{-}|$
        %& |\#total-B & \#active-B & \#inactive-B
        & $|\SetCompounds_{\scriptsize \bioassay_Q}|$
        	& $|\SetCompounds_{\scriptsize \bioassay_Q}^{+}|$ 
        	& $|\SetCompounds_{\scriptsize \bioassay_Q}^{-}|$
        	\\
        \midrule
        \endhead
        %
        \midrule
        \multicolumn{8}{|r|}{{Continued on next page}} \\
        \endfoot
        %
        \midrule
        \insertTableNotes
        \endlastfoot        
        
NP\_005021 & NP\_004705 & 20,396 & 10,198 & 10,198 & 164 & 82 & 82 \\
NP\_000903 & EAW86722 & 302 & 151 & 151 & 666 & 333 & 333 \\
NP\_000903 & BAB91222 & 302 & 151 & 151 & 166 & 83 & 83 \\
NP\_005292 & BAB91222 & 414 & 207 & 207 & 166 & 83 & 83 \\
NP\_005292 & NP\_004942 & 414 & 207 & 207 & 134 & 67 & 67 \\
NP\_004081 & NP\_002825 & 3,288 & 1,644 & 1,644 & 248 & 124 & 124 \\
NP\_997055 & NP\_004942 & 5,052 & 2,526 & 2,526 & 134 & 67 & 67 \\
NP\_775180 & ADZ17337 & 306 & 153 & 153 & 170 & 85 & 85 \\
NP\_000483 & ABD72211 & 356 & 178 & 178 & 1,188 & 594 & 594 \\
NP\_000483 & NP\_000918 & 358 & 179 & 179 & 204 & 102 & 102 \\
NP\_000483 & NP\_004818 & 358 & 179 & 179 & 178 & 89 & 89 \\
ADZ17337 & AAI28575 & 156 & 78 & 78 & 592 & 296 & 296 \\
ADZ17337 & NP\_000448 & 172 & 86 & 86 & 298 & 149 & 149 \\
ADZ17337 & NP\_066285 & 172 & 86 & 86 & 342 & 171 & 171 \\
NP\_000762 & NP\_000752 & 888 & 444 & 444 & 1,918 & 959 & 959 \\
NP\_000760 & NP\_000752 & 1,356 & 678 & 678 & 2,070 & 1,035 & 1,035 \\
NP\_002084 & P53779 & 1,358 & 679 & 679 & 112 & 56 & 56 \\
AAI28575 & P51449 & 608 & 304 & 304 & 244 & 122 & 122 \\
AAI28575 & BAH02301 & 608 & 304 & 304 & 626 & 313 & 313 \\
AAI28575 & NP\_000448 & 608 & 304 & 304 & 298 & 149 & 149 \\
AAI28575 & NP\_066285 & 610 & 305 & 305 & 346 & 173 & 173 \\
AAB26273 & NP\_000947 & 536 & 268 & 268 & 272 & 136 & 136 \\
AAB26273 & AAI27629 & 552 & 276 & 276 & 320 & 160 & 160 \\
AAB26273 & NP\_000676 & 552 & 276 & 276 & 416 & 208 & 208 \\
AAB26273 & NP\_001391 & 548 & 274 & 274 & 688 & 344 & 344 \\
AAB26273 & NP\_004358 & 552 & 276 & 276 & 116 & 58 & 58 \\
AAB26273 & NP\_000901 & 552 & 276 & 276 & 174 & 87 & 87 \\
AAB26273 & EAW86722 & 552 & 276 & 276 & 700 & 350 & 350 \\
AAB26273 & NP\_000900 & 552 & 276 & 276 & 206 & 103 & 103 \\
AAB26273 & AAH14970 & 552 & 276 & 276 & 252 & 126 & 126 \\
AAB26273 & BAB91222 & 552 & 276 & 276 & 182 & 91 & 91 \\
AAB26273 & NP\_003605 & 552 & 276 & 276 & 360 & 180 & 180 \\
AAB26273 & NP\_612200 & 552 & 276 & 276 & 542 & 271 & 271 \\
AAB26273 & NP\_001516 & 552 & 276 & 276 & 310 & 155 & 155 \\
NP\_000947 & AAI27629 & 278 & 139 & 139 & 318 & 159 & 159 \\
NP\_000947 & EAW86722 & 278 & 139 & 139 & 700 & 350 & 350 \\
NP\_000947 & BAB91222 & 278 & 139 & 139 & 182 & 91 & 91 \\
NP\_000947 & NP\_001516 & 278 & 139 & 139 & 308 & 154 & 154 \\
NP\_036559 & P00748 & 168 & 84 & 84 & 274 & 137 & 137 \\
NP\_036559 & AAC63054 & 184 & 92 & 92 & 410 & 205 & 205 \\
NP\_036559 & AAF04852 & 218 & 109 & 109 & 1,362 & 681 & 681 \\
NP\_036559 & NP\_004337 & 218 & 109 & 109 & 1,556 & 778 & 778 \\
NP\_036559 & AAA51985 & 174 & 87 & 87 & 180 & 90 & 90 \\
NP\_036559 & AAI29989 & 218 & 109 & 109 & 1,592 & 796 & 796 \\
NP\_036559 & AAH14460 & 202 & 101 & 101 & 120 & 60 & 60 \\
NP\_065717 & NP\_001387 & 1,028 & 514 & 514 & 278 & 139 & 139 \\
NP\_065717 & EAW70217 & 1,268 & 634 & 634 & 260 & 130 & 130 \\
AAI27629 & EAW86722 & 320 & 160 & 160 & 698 & 349 & 349 \\
AAI27629 & NP\_004942 & 320 & 160 & 160 & 138 & 69 & 69 \\
P00748 & NP\_660205 & 320 & 160 & 160 & 1,586 & 793 & 793 \\
P00748 & NP\_004521 & 320 & 160 & 160 & 214 & 107 & 107 \\
P00748 & AAC63054 & 266 & 133 & 133 & 382 & 191 & 191 \\
P00748 & AAF04852 & 320 & 160 & 160 & 1,364 & 682 & 682 \\
P00748 & NP\_004337 & 320 & 160 & 160 & 1,558 & 779 & 779 \\
P00748 & AAA51985 & 244 & 122 & 122 & 154 & 77 & 77 \\
P00748 & AAI29989 & 320 & 160 & 160 & 1,596 & 798 & 798 \\
P00748 & AAH14460 & 296 & 148 & 148 & 114 & 57 & 57 \\
ABD72211 & NP\_000918 & 1,210 & 605 & 605 & 202 & 101 & 101 \\
ABD72211 & NP\_004818 & 1,210 & 605 & 605 & 178 & 89 & 89 \\
AAH04460 & AAH14460 & 890 & 445 & 445 & 138 & 69 & 69 \\
NP\_000676 & NP\_005152 & 154 & 77 & 77 & 172 & 86 & 86 \\
NP\_000676 & NP\_000901 & 416 & 208 & 208 & 176 & 88 & 88 \\
NP\_000676 & EAW86722 & 418 & 209 & 209 & 700 & 350 & 350 \\
NP\_000676 & NP\_001516 & 418 & 209 & 209 & 310 & 155 & 155 \\
NP\_000676 & NP\_004942 & 418 & 209 & 209 & 138 & 69 & 69 \\
NP\_005152 & NP\_004358 & 512 & 256 & 256 & 108 & 54 & 54 \\
NP\_005152 & NP\_001516 & 518 & 259 & 259 & 310 & 155 & 155 \\
NP\_001391 & NP\_000901 & 682 & 341 & 341 & 174 & 87 & 87 \\
NP\_001391 & EAW86722 & 690 & 345 & 345 & 700 & 350 & 350 \\
NP\_001391 & NP\_000900 & 682 & 341 & 341 & 206 & 103 & 103 \\
NP\_001391 & BAB91222 & 690 & 345 & 345 & 182 & 91 & 91 \\
NP\_001391 & NP\_001516 & 690 & 345 & 345 & 308 & 154 & 154 \\
NP\_660205 & NP\_004337 & 914 & 457 & 457 & 642 & 321 & 321 \\
NP\_660205 & AAI29989 & 986 & 493 & 493 & 642 & 321 & 321 \\
NP\_005424 & NP\_001387 & 736 & 368 & 368 & 540 & 270 & 270 \\
NP\_005424 & NP\_003984 & 736 & 368 & 368 & 166 & 83 & 83 \\
NP\_005424 & NP\_004705 & 736 & 368 & 368 & 164 & 82 & 82 \\
NP\_005424 & NP\_004062 & 736 & 368 & 368 & 176 & 88 & 88 \\
AAC63054 & AAF04852 & 446 & 223 & 223 & 1,364 & 682 & 682 \\
AAC63054 & NP\_004337 & 446 & 223 & 223 & 1,558 & 779 & 779 \\
AAC63054 & AAA51985 & 402 & 201 & 201 & 182 & 91 & 91 \\
AAC63054 & AAI29989 & 446 & 223 & 223 & 1,594 & 797 & 797 \\
AAC63054 & AAH14460 & 438 & 219 & 219 & 130 & 65 & 65 \\
AAF04852 & NP\_004337 & 654 & 327 & 327 & 718 & 359 & 359 \\
AAF04852 & AAI29989 & 682 & 341 & 341 & 696 & 348 & 348 \\
NP\_004337 & AAI29989 & 804 & 402 & 402 & 758 & 379 & 379 \\
AAA51985 & AAI29989 & 210 & 105 & 105 & 1,598 & 799 & 799 \\
AAA51985 & AAH14460 & 194 & 97 & 97 & 118 & 59 & 59 \\
NP\_004358 & NP\_000901 & 116 & 58 & 58 & 176 & 88 & 88 \\
NP\_004358 & EAW86722 & 116 & 58 & 58 & 700 & 350 & 350 \\
NP\_004358 & NP\_000900 & 116 & 58 & 58 & 208 & 104 & 104 \\
NP\_004358 & AAH14970 & 116 & 58 & 58 & 244 & 122 & 122 \\
NP\_004358 & BAB91222 & 116 & 58 & 58 & 182 & 91 & 91 \\
NP\_004358 & NP\_001516 & 116 & 58 & 58 & 312 & 156 & 156 \\
NP\_004221 & EAW86722 & 138 & 69 & 69 & 700 & 350 & 350 \\
NP\_004221 & NP\_001516 & 138 & 69 & 69 & 312 & 156 & 156 \\
NP\_004221 & NP\_004942 & 138 & 69 & 69 & 138 & 69 & 69 \\
NP\_000901 & EAW86722 & 174 & 87 & 87 & 700 & 350 & 350 \\
NP\_000901 & BAB91222 & 176 & 88 & 88 & 182 & 91 & 91 \\
NP\_000901 & NP\_001516 & 176 & 88 & 88 & 312 & 156 & 156 \\
EAW86722 & AAH14970 & 700 & 350 & 350 & 250 & 125 & 125 \\
EAW86722 & BAB91222 & 700 & 350 & 350 & 182 & 91 & 91 \\
EAW86722 & NP\_001516 & 700 & 350 & 350 & 312 & 156 & 156 \\
NP\_000900 & BAB91222 & 208 & 104 & 104 & 182 & 91 & 91 \\
NP\_000900 & NP\_001516 & 208 & 104 & 104 & 312 & 156 & 156 \\
NP\_000900 & NP\_004942 & 208 & 104 & 104 & 138 & 69 & 69 \\
AAH14970 & BAB91222 & 252 & 126 & 126 & 182 & 91 & 91 \\
AAH14970 & NP\_001516 & 252 & 126 & 126 & 310 & 155 & 155 \\
AAH14970 & NP\_004942 & 252 & 126 & 126 & 138 & 69 & 69 \\
NP\_002721 & NP\_001387 & 142 & 71 & 71 & 540 & 270 & 270 \\
NP\_002721 & NP\_003984 & 142 & 71 & 71 & 166 & 83 & 83 \\
NP\_002721 & NP\_004705 & 142 & 71 & 71 & 164 & 82 & 82 \\
NP\_002721 & NP\_004062 & 142 & 71 & 71 & 176 & 88 & 88 \\
BAB91222 & NP\_004942 & 182 & 91 & 91 & 138 & 69 & 69 \\
NP\_003605 & NP\_004942 & 362 & 181 & 181 & 138 & 69 & 69 \\
NP\_001387 & EAW70217 & 488 & 244 & 244 & 260 & 130 & 130 \\
EAW70217 & NP\_003984 & 278 & 139 & 139 & 136 & 68 & 68 \\
EAW70217 & NP\_004705 & 280 & 140 & 140 & 132 & 66 & 66 \\
EAW70217 & NP\_004062 & 280 & 140 & 140 & 142 & 71 & 71 \\
NP\_001124480 & NP\_002825 & 128 & 64 & 64 & 318 & 159 & 159
%
\end{longtable}
\end{ThreePartTable}

==> tables/supp_final_bioassay_stat.tex <==
\begin{ThreePartTable}
\centering
\begin{TableNotes}
\item In this table, the columns protacxn, \#total, \#active and \#inactive correspond to the target protein's accession number from PubChem, number of total compounds, active compounds and inactive compounds in the bioassay, respectively.
The column Protein family denotes the corresponding protein family for each target.
\par
\end{TableNotes}


\begin{longtable}[h]
		{
		@{\hspace{5pt}}c@{\hspace{5pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{2pt}}r@{\hspace{2pt}}
		@{\hspace{10pt}}c@{\hspace{10pt}}
		}
		
		\caption{Compound statistics of processed bioassays}
		\label{tbl:supp:final_bio_stat} \\
		%
		\midrule
        	protacxn & \#total & \# active &  \# inactive & Protein family\\ 
        \midrule
        \endfirsthead
        %
        
        \multicolumn{5}{c}%
        {{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
	%
	\midrule
        	protacxn & \#total & \# active &  \# inactive  & Protein family\\ 
        \midrule
        \endhead
        %
        \midrule
        \multicolumn{5}{|r|}{{Continued on next page}} \\
        \endfoot
        %
        \midrule
        \insertTableNotes
        \endlastfoot
        %
        NP\_001017535 & 380,711 & 5,152 & 375,559 & Nuclear hormone receptor family \\
AAH18745 & 374,923 & 1,230 & 373,693 & Peptidase family \\
NP\_005021 & 349,900 & 10,198 & 339,702 & Protein kinase superfamily \\
NP\_004196 & 336,578 & 238 & 336,340 & Peptidase family \\
NP\_057051 & 292,415 & 97 & 292,318 & Protein-tyrosine phosphatase family \\
NP\_000903 & 292,382 & 151 & 292,231 & G-protein coupled receptor 1 family \\
NP\_005292 & 292,044 & 207 & 291,837 & G-protein coupled receptor 1 family \\
NP\_004081 & 290,998 & 1,674 & 289,324 & Protein-tyrosine phosphatase family \\
NP\_001121649 & 275,994 & 116 & 275,878 & Nuclear hormone receptor family \\
NP\_997055 & 208,843 & 2,526 & 206,317 & G-protein coupled receptor 1 family \\
NP\_002736 & 182,123 & 1,207 & 180,916 & Protein kinase superfamily \\
NP\_542155 & 112,687 & 906 & 111,781 & Protein-tyrosine phosphatase family \\
NP\_775180 & 96,456 & 153 & 96,303 & Nuclear hormone receptor family \\
P55210 & 71,790 & 77 & 71,713 & Peptidase family \\
NP\_150634 & 70,986 & 61 & 70,925 & Peptidase family \\
NP\_000483 & 10,100 & 179 & 9,921 & ABC transporter superfamily \\
%NP\_001308829 & 7,266 & 233 & 7,033 & Histone deacetylase family \\
ABB72139 & 6,968 & 64 & 6,904 & Nuclear hormone receptor family \\
ADZ17337 & 6,738 & 86 & 6,652 & Nuclear hormone receptor family \\
NP\_000762 & 7,759 & 1,163 & 6,596 & Cytochrome P450 family \\
EAW77416 & 7,131 & 626 & 6,505 & Cytochrome P450 family \\
ADZ17384 & 6,425 & 55 & 6,370 & Nuclear hormone receptor family \\
NP\_000760 & 7,676 & 1,713 & 5,963 & Cytochrome P450 family \\
NP\_000752 & 7,670 & 4,008 & 3,662 & Cytochrome P450 family \\
AAF64255 & 2,728 & 1,107 & 1,621 & Bcl-2 family \\
NP\_002084 & 2,285 & 682 & 1,603 & Protein kinase superfamily \\
NP\_063937 & 2,390 & 823 & 1,567 & Protein kinase superfamily \\
AAI28575 & 1,824 & 305 & 1,519 & Nuclear hormone receptor family \\
AAB26273 & 1,669 & 276 & 1,393 & G-protein coupled receptor 1 family \\
NP\_000947 & 1,350 & 139 & 1,211 & G-protein coupled receptor 1 family \\
NP\_036559 & 1,260 & 109 & 1,151 & Peptidase family \\
NP\_065717 & 1,630 & 661 & 969 & Protein kinase superfamily \\
AAI27629 & 1,065 & 160 & 905 & G-protein coupled receptor 1 family \\
P51449 & 978 & 138 & 840 & Nuclear hormone receptor family \\
NP\_004040 & 824 & 91 & 733 & Bcl-2 family \\
P00748 & 761 & 160 & 601 & Peptidase family \\
ABD72211 & 1,164 & 605 & 559 & ABC transporter superfamily \\
AAH04460 & 993 & 445 & 548 & Peptidase family \\
NP\_004950 & 954 & 456 & 498 & Nuclear hormone receptor family \\
NP\_000676 & 667 & 209 & 458 & G-protein coupled receptor 1 family \\
NP\_000466 & 489 & 55 & 434 & Nuclear hormone receptor family \\
NP\_005152 & 672 & 259 & 413 & G-protein coupled receptor 1 family \\
NP\_001391 & 729 & 345 & 384 & G-protein coupled receptor 1 family \\
NP\_005217 & 456 & 82 & 374 & G-protein coupled receptor 1 family \\
NP\_660205 & 1,167 & 795 & 372 & Peptidase family \\
NP\_000789 & 457 & 100 & 357 & G-protein coupled receptor 1 family \\
NP\_001027450 & 543 & 203 & 340 & Peptidase family \\
NP\_004521 & 445 & 107 & 338 & Peptidase family \\
NP\_004960 & 387 & 61 & 326 & Peptidase family \\
NP\_005424 & 693 & 368 & 325 & Protein kinase superfamily \\
P53779 & 362 & 57 & 305 & Protein kinase superfamily \\
AAC63054 & 517 & 223 & 294 & Peptidase family \\
AAF04852 & 973 & 683 & 290 & Peptidase family \\
NP\_004337 & 1,055 & 781 & 274 & Peptidase family \\
AAA51985 & 366 & 105 & 261 & Peptidase family \\
NP\_004358 & 289 & 58 & 231 & G-protein coupled receptor 1 family \\
NP\_004221 & 276 & 69 & 207 & G-protein coupled receptor 1 family \\
NP\_000901 & 292 & 88 & 204 & G-protein coupled receptor 1 family \\
NP\_002522 & 349 & 156 & 193 & G-protein coupled receptor 1 family \\
NP\_644806 & 248 & 57 & 191 & Peptidase family \\
EAW86722 & 539 & 350 & 189 & G-protein coupled receptor 1 family \\
NP\_000900 & 291 & 104 & 187 & G-protein coupled receptor 1 family \\
AAI07736 & 242 & 59 & 183 & Bcl-2 family \\
AAI29989 & 981 & 799 & 182 & Peptidase family \\
BAH02301 & 462 & 317 & 145 & Nuclear hormone receptor family \\
NP\_000448 & 292 & 149 & 143 & Nuclear hormone receptor family \\
NP\_004841 & 229 & 88 & 141 & Protein kinase superfamily \\
AAH14970 & 248 & 126 & 122 & G-protein coupled receptor 1 family \\
NP\_002721 & 190 & 71 & 119 & Protein kinase superfamily \\
NP\_003813 & 211 & 92 & 119 & Nuclear hormone receptor family \\
AAH36651 & 210 & 92 & 118 & Protein kinase superfamily \\
Q05397 & 210 & 110 & 100 & Protein kinase superfamily \\
NP\_004570 & 151 & 52 & 99 & Protein kinase superfamily \\
NP\_000918 & 189 & 102 & 87 & ABC transporter superfamily \\
NP\_112168 & 304 & 217 & 87 & Protein kinase superfamily \\
NP\_066285 & 233 & 173 & 60 & Nuclear hormone receptor family \\
BAB91222 & 142 & 91 & 51 & G-protein coupled receptor 1 family \\
NP\_003605 & 232 & 181 & 51 & G-protein coupled receptor 1 family \\
P28566 & 95 & 51 & 44 & G-protein coupled receptor 1 family \\
NP\_037457 & 331 & 290 & 41 & Peptidase family \\
Q6L5J4 & 432 & 391 & 41 & G-protein coupled receptor 1 family \\
NP\_000732 & 98 & 58 & 40 & G-protein coupled receptor 1 family \\
NP\_612200 & 314 & 274 & 40 & G-protein coupled receptor 1 family \\
NP\_001387 & 307 & 270 & 37 & Protein kinase superfamily \\
NP\_004818 & 125 & 89 & 36 & ABC transporter superfamily \\
EAW70217 & 188 & 154 & 34 & Protein kinase superfamily \\
AAH14460 & 91 & 69 & 22 & Peptidase family \\
NP\_001124480 & 81 & 64 & 17 & Protein-tyrosine phosphatase family \\
NP\_001516 & 171 & 156 & 15 & G-protein coupled receptor 1 family \\
%AAI30529 & 64 & 50 & 14 & G-protein coupled receptor 3 family \\
NP\_003984 & 95 & 83 & 12 & Protein kinase superfamily \\
NP\_004705 & 94 & 82 & 12 & Protein kinase superfamily \\
NP\_004062 & 96 & 88 & 8 & Protein kinase superfamily \\
NP\_002825 & 166 & 160 & 6 & Protein-tyrosine phosphatase family \\
NP\_004942 & 74 & 69 & 5 & G-protein coupled receptor 1 family
	%
\end{longtable}
\end{ThreePartTable}

==> tables/topn_task.tex <==
\begin{table}[h]
\centering
\caption{Top-$N$ Performance Comparison (\%)}
\label{tbl:topn_task}
\begin{small}
  \begin{threeparttable}
      \begin{tabular}{
          @{\hspace{10pt}}l@{\hspace{10pt}}
          @{\hspace{10pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
          @{\hspace{10pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
%          @{\hspace{5pt}}r@{\hspace{5pt}}
          @{\hspace{10pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
          @{\hspace{5pt}}r@{\hspace{5pt}}
          }
          %
          \toprule
          {method} 
          & \multicolumn{3}{c}{\rocauc} 
          & \multicolumn{3}{c}{\prauc} 
%          & \multicolumn{3}{c}{\precision} 
%          & \multicolumn{3}{c}{\sensitivity} 
%          & \multicolumn{3}{c}{\tnr} 
%          & \multicolumn{3}{c}{\accuracy} 
          & \multicolumn{3}{c}{\fone} 
          \\
          \cmidrule(lr){1-1}
          \cmidrule(lr){2-4}
          \cmidrule(lr){5-7}
          \cmidrule(lr){8-10}
%          \cmidrule(lr){11-13}
%          \cmidrule(lr){14-16}
%          \cmidrule(lr){17-19}
%          \cmidrule(lr){20-22}
          top-$N$ & 1 & 3 & 5
          & 1 & 3 & 5
%          & 1 & 3 & 5
%          & 1 & 3 & 5
%         & 1 & 3 & 5
%          & 1 & 3 & 5
          & 1 & 3 & 5
          \\
          \midrule
		 \morganFCN & 10 &  15 &  20 
		 & 13 &  21 &  30 
%		 & 4 &  8 &  15 
%		 & 7 &  20 &  28 
%		 & 4 &  7 &  12 
%		 & 10 &  18 &  22 
		 & 11 &  19 &  23 
		 \\
		 \morgancFCN & 2 &  13 &  18 
		 & 3 &  17 &  22 
%		 & 2 &  9 &  16 
%		 & 2 &  15 &  23 
%		 & 1 &  8 &  14 
%		 & 5 &  16 &  21 
		 & 4 &  17 &  22
		 \\
		 \dmpnnFCN & 5 &  9 &  17 
		 & 6 &  11 &  17 
%		 & 0 &  1 &  5 
%		 & 36 &  66 &  72 
%		 & 3 &  6 &  16 
%		 & 3 &  6 &  17 
		 & 10 &  19 &  30
		 \\
		 \newgnnFCN & 4 &  10 &  26 
		 & 2 &  7 &  20 
%		 & 4 &  8 &  16 
%		 & 15 &  31 &  42 
%		 & 7 &  15 &  23 
%		 & 1 &  4 &  17 
		 & 5 &  11 &  26
		 \\
		 \dmpnnFCNDT & 2 &  11 &  23 
		 & 4 &  13 &  24 
%		 & 3 &  10 &  19 
%		 & 12 &  24 &  35 
%		 & 7 &  15 &  28 
%		 & 2 &  8 &  20 
		 & 5 &  13 &  22
		 \\
		 \newgnnFCNDT & 5 &  18 &  33 
		 & 6 &  14 &  31 
%		 & 8 &  22 &  46 
%		 & 2 &  17 &  31 
%		 & 12 &  31 &  49 
%		 & 2 &  8 &  25 
		 & 2 &  8 &  23
		 \\
		 \midrule
		 \DANNWithDMPNN & 2 &  9 &  16 
		 & 1 &  5 &  15 
%		 & 10 &  23 &  34 
%		 & 12 &  23 &  31 
%		 & 15 &  38 &  50 
%		 & 3 &  8 &  20 
		 & 3 &  10 &  19 
		 \\
		 \DANNWithDMPNNA 
		 & 2 &  8 &  17 
		 & 1 &  8 &  15 
%		 & 9 &  20 &  29 
%		 & 5 &  21 &  30 
%		 & 13 &  31 &  44 
%		 & 4 &  7 &  16 
		 & 2 &  11 &  19
		 \\
		 \midrule
		\OurMethodWithDMPNN 
		& 18 &  52 &  85 
		& 17 &  48 &  81 
%		& 11 &  37 &  74 
%		& 4 &  17 &  48 
%		& 3 &  23 &  57 
%		& 21 &  57 &  90 
		& 12 &  49 &  \textbf{81}
		\\
		\OurMethodWithDMPNNWithDisc 
		& 12 &  45 &  79 
		& 15 &  48 &  80 
%		& 20 &  53 &  85 
%		& 8 &  32 &  68 
%		& 15 &  49 &  75 
%		& 18 &  60 &  88 
		& \textbf{17} &  \textbf{50} &  80
		\\
		\OurMethodWithDMPNNA 
		&  \textbf{22} &  \textbf{62} &  \textbf{89} 
		& 14 &  55 &  83 
%		& 9 &  48 &  78 
%		& 4 &  17 &  43 
%		& 6 &  31 &  63 
%		& 18 &  60 &  87 
		& 13 &  43 &  78
		\\
		\OurMethodWithDMPNNAWithDisc 
		& 16 &  51 &  81 
		& \textbf{20} &  \textbf{56} &  \textbf{86} 
%		& 22 &  61 &  87 
%		& 6 &  32 &  69 
%		& 18 &  52 &  77 
%		& 14 &  55 &  88 
		& 15 &  \textbf{50} &  \textbf{81}
		\\
	\bottomrule
	\end{tabular}
	%

	\begin{tablenotes}
        \setlength\labelsep{0pt}
		\begin{footnotesize}
		\item In this table, the columns \rocauc, \prauc,
		%\precision,\sensitivity, \tnr, \accuracy, 
		and \fone have the percentage of tasks
		for which each method is ranked within the top-1, top-3 and top-5 best methods 
		in respective metrics.
		The best performance values are \textbf{boldfaced}. 
		\par
		\end{footnotesize}
	\end{tablenotes}

\end{threeparttable}
\end{small}
\end{table}
